The SMART approach to instance-optimal online learning

We devise an online learning algorithm -- titled Switching via Monotone Adapted Regret Traces (SMART) -- that adapts to the data and achieves regret that is instance optimal, i.e., simultaneously competitive on every input sequence compared to the performance of the follow-the-leader (FTL) policy and the worst case guarantee of any other input policy. We show that the regret of the SMART policy on any input sequence is within a multiplicative factor $e/(e-1) \approx 1.58$ of the smaller of: 1) the regret obtained by FTL on the sequence, and 2) the upper bound on regret guaranteed by the given worst-case policy. This implies a strictly stronger guarantee than typical `best-of-both-worlds' bounds as the guarantee holds for every input sequence regardless of how it is generated. SMART is simple to implement as it begins by playing FTL and switches at most once during the time horizon to the worst-case algorithm. Our approach and results follow from an operational reduction of instance optimal online learning to competitive analysis for the ski-rental problem. We complement our competitive ratio upper bounds with a fundamental lower bound showing that over all input sequences, no algorithm can get better than a $1.43$-fraction of the minimum regret achieved by FTL and the minimax-optimal policy. We also present a modification of SMART that combines FTL with a ``small-loss" algorithm to achieve instance optimality between the regret of FTL and the small loss regret bound.

==> arxiv/arxiv_body/CoverResult_arxiv.tex <==
\section{Fundamental limits of binary prediction: Cover's result} \label{appendix:Cover}

In the setting of binary prediction, the remarkable result of~\cite{Cover1966} stated next provides an exact characterization of the set of all loss functions achievable in binary prediction. This result equips us with the \emph{exact} minmax optimal algorithm for binary prediction alluded to in Section~\ref{sec:intro}, as well equips us with other tools we employ later. 
\begin{theorem}  \label{thm:CoverAchievableFn}
A loss function $\phi : \{0,1\}^n \to \mathbb{R}^+$ be \emph{achievable} in binary prediction if there exists a predictor/strategy $a_t: y^{t-1} \mapsto [0,1]$ that achieves $\sum_{t=1}^n |a_t(y^{t-1})-y_t| = \phi(y^n)$ 
for all $y^n$. Then, $\phi$ is achievable if and only if it satistfies the following two conditions:
\begin{itemize}
    \item Balance: For $\e^n \sim \mathrm{Bern}\left(\frac{1}{2}\right)$ i.i.d.,  $\E[\phi(Y^n)] = \frac{n}{2}$ . 
    \item Stability: Let $\phi_t(y^t) \equiv \E[\phi(y^{t}\e_{t+1}^n)]$ where $\e_{t+1}^n \sim \mathrm{Bern}\left(\frac{1}{2}\right)$ i.i.d. Then $|\phi_t(y^{t-1}0)-\phi_t(y^{t-1}1)| \le 1$. 
    \end{itemize}
    Furthermore, if a function $\phi$ is satisfies the above two conditions, then the predictor $a_t(y^{t-1}) = \frac{1+\phi_t(y^{t-1}0)-\phi_t(y^{t-1}1)}{2}$ achieves it.
\end{theorem}

An illuminating question is whether the loss of the hindsight-optimal action, i.e. $\phi(y^n) = \min\{\sum_{t=1}^n y_i, n-\sum_{t=1}^n y_i\}$ is achievable, which is answered in the negative by Cover's result. 

\begin{corollary} \label{cor:BinPredOptReg}
    The loss function $y^n \mapsto \min\left\{\sum_{t=1}^n y_i, n-\sum_{t=1}^n y_i\right\}$ violates the balance condition and therefore is not achievable. However, the function 
    \begin{align}
    \label{eq:CoverLossFn}
    y^n \mapsto \min\left\{\sum_{t=1}^n y_i, n-\sum_{t=1}^n y_i\right\} + \frac{\E|\sum_{t=1}^n Z_t|}{2}
    \end{align}
    where $Z^n \sim \Unif\{+1,-1\}$ i.i.d. is achievable. The predictor that achieves~\cref{eq:CoverLossFn} chooses $\widehat{Y}_t$ (equivalently, $a_t = \mathsf{P}[\widehat{Y_t} = 1]$) as
        $\widehat{Y}_t = \Majority\{y^{t-1},\e_{t+1}^n\}$
    where $\e_{t+1}^n \sim \mathrm{Bern}\left(\frac{1}{2}\right)$ i.i.d., with ties broken uniformly at random. Finally, Cover's predictor is \emph{minmax optimal} in the sense that for any other predictor $\alg$, 
    \[
    \max_{y^n} \Reg(\alg, y^n) \ge \max_{y^n} \Reg(\Cover, y^n) = \sqrt{\frac{n}{2\pi}}(1+o(1))
    \]
\end{corollary}

==> arxiv/arxiv_body/ftl_arxiv.tex <==
\subsection{A Regret Decomposition for $\ftl$} 
\label{ssec:FTL}

Our results rely on the following regret decomposition for the $\ftl$ policy in any online learning setting. This decomposition was first introduced in~\cite[Section 3]{kalai2005efficient}, and is well-known in the literature, where it is often referred to as the `be-the-leader lemma'. \abcomment{Kalai--Vempala doesn't have this regret equality for FTL, does it?.. Actually I don't think I have this regret equality result before when people use the be the leader lemma} We note in particular that Lemma~\ref{lem:FTLRegret} requires no assumptions on the loss function such as boundedness and convexity. 

\begin{lemma}[Regret of $\ftl$] \label{lem:FTLRegret}
If $L_t(\cdot) \defeq \sum_{i=1}^t \ell_t(\cdot)$, i.e. the cumulative loss function, then
\begin{align} \label{eq:FTLRegEquality}
    \Reg(\ftl, \ell^n) = \sum_{t=1}^n (L_t(a^*_{t-1}) - L_t(a^*_t)). 
\end{align}
  % \begin{itemize}
  %       \item (OCO) If $\ell_t(\cdot)$ is strictly convex (implying that a unique minimizer in~\cref{eq:HindsightOPTdef} exists) then 
  %       \begin{align} \label{eq:FTLRegOCO}
  %           \Reg(\ftl, \ell^n) = \textstyle\sum_{t=1}^n (L_t(a^*_{t-1}) - L_t(a^*_t))
  %       \end{align}
  %       \item (Prediction with experts) Recall the problem defined in~\cref{eq:PWERegDef}. In this case, 
  %       \begin{align*}%\label{eq:RegPWEFTL}
  %           \Reg(\ftl,\ell^n) = \textstyle\sum_{t=1}^n (u_{j^*_{t-1}}^T L_t - u_{j^*_{t}}^T L_t)
  %       \end{align*}
  %   \end{itemize} 
\end{lemma}

% \begin{proof}
%     We establish the result for the OCO case---the proof is identical for PWE. Recalling $\aftl_t = a^*_{t-1}$ we have 
%     \begin{align*}
%         \Reg(\ftl, \ell^n) &= \sum_{t=1}^n \ell_t(a^*_{t-1})  - \inf_{a \in \Ac} \sum_{t=1}^n \ell_t(a) \\
%         &= \sum_{t=1}^n \ell_t(a^*_{t-1})  - L_n(a^*_n) \\
%         &= \sum_{t=1}^n (L_t(a^*_{t-1}) - L_{t-1}(a^*_{t-1})) -  L_n(a^*_n) \\
%         &= \sum_{t=1}^n (L_t(a^*_{t-1}) - L_t(a^*_t)) + \sum_{t=1}^n (L_t(a^*_t) - L_{t-1}(a^*_{t-1})) - L_n(a^*_n) \\
%         &\stackrel{(a)}{=} \sum_{t=1}^n (L_t(a^*_{t-1}) - L_t(a^*_t))
%     \end{align*}
%     where $(a)$ follows since $\sum_{t=1}^n (L_t(a^*_t) - L_{t-1}(a^*_{t-1})) = L_n(a^*_n)$ by a telescoping sum. 
% \end{proof}

Upon instantiating the regret bound obtained in~\cref{lem:FTLRegret} for binary prediction, we observe that the $\ftl$ regret admits a geometric interpretation. 
\begin{definition}[Line crossings]\label{defn:StateLineCross}
    For $y_1^n\in\{0,1\}^n$, let  $S_t(y^t) = \textstyle\sum_{i=1}^t y_i - (t-\textstyle\sum_{i=1}^t y_i) = 2\textstyle\sum_{i=1}^t y_i - t$. 
 For any $t$, 
%  \begin{align*}
% %\label{eq:NumCrossingsDefn}
     $c(y^t) \defeq \left|\left\{0 \le j \le t | S_j = 0\right\}\right|$,
     % \end{align*}
 and each $j$ such that $S_j = 0$ is called a line crossing. 
\end{definition}

\begin{corollary}[$\ftl$ for binary prediction] \label{cor:BinPred}
    In binary prediction,
    %\label{eq:BinPredReg}[]
        $\Reg(\ftl, y^n) = \frac{c(y^{n-1})}{2}.$
\end{corollary}
% \begin{proof}
%     Follows from~\cref{eq:RegPWEFTL}, since the sum in the RHS is zero if $t-1$ is not a line crossing, and is $\frac{1}{2}$ when $t-1$ is a line crossing. 
% \end{proof}


==> arxiv/arxiv_body/mainresults_arxiv.tex <==
\subsection{Main results} \label{ssec:mainresults}

==> arxiv/arxiv_body/setting_arxiv.tex <==
\section{Setting and Preliminaries}
\label{ssec:setting}

%We formally describe the general online learning setting and the $\ftl$ algorithm in such settings.

%\subsection{Online Learning, Regret, and Instance Optimality}

We consider a general online learning problem with horizon of $n$ rounds: at the start of each round $t \in [n]$, a policy $\alg$ first plays an action $a_t$ from some action set $\Ac$, following which, a loss function $\ell_t: \Ac \to [0,1]$ is revealed, resulting in a loss of $\ell_t(a_t)$. 
The aim is to minimize the \emph{regret} (i.e., additive loss) compared to the best fixed action in hindsight:
\begin{align}
\label{eq:RegDefnGeneral}
    \Reg(\alg,\ell^n) = \textstyle\sum_{t=1}^n \ell_t(a_t) - \inf_{a \in \Ac} \textstyle\sum_{t=1}^n \ell_t(a).
\end{align} 
While the setting can be defined over general action set $\Ac$ and additive loss functions $\ell_t(\cdot)$, the most common case considered  is that online convex optimization (OCO), where the action set $\Ac$ is convex, and loss functions $\ell_t(\cdot)$ are convex and bounded. 
% Given loss functions $\ell^{t}$, the hindsight optimal action is defined as  
% \begin{align} \label{eq:HindsightOPTdef}
%     a^*_t \defeq \argmin_{a \in \Ac} \textstyle\sum_{i=1}^{t} \ell_i(a) 
% \end{align}
% where we note that the right hand side of~\cref{eq:HindsightOPTdef} might be a set if multiple minimizers exist.
Given the above setting, one performance measure of an algorithm is the \emph{worst-case} regret $\Reg(\alg) \defeq \sup_{\ell^n} \Reg(\alg,\ell^n)$. 
A low (sublinear) worst-case regret ensures outcomes are robust to inputs. On the other hand, if the $\ell_t$ are stochastic -- in particular, drawn i.i.d. from a fixed (unknown) distribution $\dist$ -- then a reasonable figure of merit is the \emph{pseudoregret}
\begin{align*} %\label{eq:DefpseudoReg}
    \PseudoReg(\alg) \defeq \sup_{\dist}\Big(\textstyle\sum_{t=1}^n \E[\ell_t(a_t)] - \inf_{a \in \Ac} \textstyle\sum_{t=1}^n \E[\ell_t(a)]\Big)
\end{align*}
\cite{kotlowski2018minimaxity}

\sbcomment{Need some segue here}
Next, we review the follow the leader (FTL) strategy and establish its regret. 
\begin{definition}[$\ftl$] \label{def:FTL}
Given loss functions $\ell^{t}$, the hindsight optimal action is defined as  
\begin{align} \label{eq:HindsightOPTdef}
    a^*_t \defeq \argmin_{a \in \Ac} \textstyle\sum_{i=1}^{t} \ell_i(a) 
\end{align}
where we note that the right hand side of~\cref{eq:HindsightOPTdef} might be a set if multiple minimizers exist. 
Then, the $\ftl$ action $a^{\mathsf{FTL}}_t = a^*_{t-1}$ with ties broken \abedit{according to an arbitrary rule.}
\end{definition}

A canonical example of an online learning problem is that of \emph{prediction with expert advice}. This is the setting where the action set $\Ac = \Delta^{m-1}$ and the loss function is of the form (with slight abuse of notation) $\ell_t(a) = a^T \ell_t$ for a vector $\ell_t \in \mathbb{R}^m_{+}$. Therefore, the problem can be interpreted as assigning a weight over $m$ experts at each time step in order to achieve low regret against the best fixed expert in hindsight, with regret given by
\begin{align}\label{eq:PWERegDef}
    \Reg(\alg,\ell^n) = \textstyle\sum_{t=1}^n a_t^T \ell_t - \min_{j \in [m]} \textstyle\sum_{t=1}^n \ell_{tj}
\end{align}
since $\min_{a \in \Delta^{m-1}} a^T\left(\sum_{t=1}^n \ell_t \right)$ always occurs at a corner point of the simplex. \abedit{Then, we set}
\begin{align} \label{eq:FTLPWEDef}
    \aftl_t =  u_{j^*_{t-1}} \defeq \Unif({j^*_{t-1}})
    ~\text{ where }
    j^*_{t} \defeq \argmin_{j \in [m]} \textstyle\sum_{i=1}^{t} \ell_{ij},
 \end{align}
i.e. $\ftl$ chooses the expert that has incurred the least loss so far, breaking ties uniformly at random.  
A special case of this setting is the binary prediction problem from~\cref{sec:intro}, where recall $\ftl$ chooses $\widehat{Y}_t = \mathsf{Majority}(y^{t-1})$, with $\widehat{Y}_t \sim \mathrm{Bern}(1/2)$ in case of a tie. 
%, where given the sequence so far $y^{t-1}, \ftl$ chooses
% \begin{align}\label{eq:binpredRegDef}
%     \Reg(\alg, y^n) = \sum_{t=1}^n |a_t - y_t| - \min\left\{\sum_{t=1}^n y_t, n - \sum_{t=1}^n y_t\right\}.
% \end{align}
% In this case, FTL chooses 
% \begin{align} \label{eq:BinFTL}
% \aftl_t = a^*_{t-1} =
% \begin{cases}
%     0 & \text{if Majority}\{y_1,\dotsc,y_{t-1}\} = 0 \\
%     1 & \text{if Majority}\{y_1,\dotsc,y_{t-1}\} = 1 \\
%     \frac{1}{2} & \text{otherwise}.
% \end{cases}
% \end{align}


Typically, algorithms and guarantees differ starkly for these two cases---optimal worst-case algorithms (henceforth $\wcalg$) typically have similar worst-case regret and pseudoregret, whereas optimal algorithms for stochastic inputs such as $\ftl$ have much lower pseudoregret, but can have much higher regret on adversarial inputs. 
Best-of-both-worlds policies aim to bridge these two by adapting to the input to achieve regret which is both within constant factor of the pseudoregret of $\ftl$ on stochastic inputs, and within constant factor of a worst-case bound on the regret of $\wcalg$.

A stronger objective is to devise an algorithm $\alg$, that on \emph{every} input $\ell^n$ is within a constant factor of the minimum of the regret of $\ftl$ and the regret of $\wcalg$ on any given input.
However, showing such a property requires the ability to understand the fine-grained performance of $\wcalg$ on any given input, which is often not possible. Thus we consider a slightly weaker variant of \emph{instance optimality} with respect to the regret of $\ftl$ and a regret upper bound $g(n)$ as stated in Definition \ref{def:instanceopt_wc}. In particular, for a regret bound $g(n)$ such that $\Reg(\wcalg, \ell^n) \leq g(n)$ for all $\ell^n$, we desire $\alg$ to satisfy
\begin{align} 
\label{eq:instoptdef}
    \Reg(\alg,\ell^n)
    \le
    \gamma\min\Big\{\Reg(\ftl, \ell^n), g(n)\Big\}
    %replaced \sup_{\tilde{\ell}^n}\big(\Reg(\wcalg, \tilde{\ell}^n)\big) with g(n)
\end{align}
for some absolute constant $\gamma$. We reiterate that such a guarantee entails a constant factor guarantee on the minimum \emph{regret} rather than the minimum \emph{loss}.
%We also note that while Eq.~\cref{eq:instanceopt} is not truly instance-optimal (in that we are comparing against the worst-case regret bound for $\wcalg$ rather than the regret on instance $\ell^n$), the two are the same if $\wcalg$ is the true minimax optimal algorithm for a given setting \abcomment{is the minmax opt always an equalizer?} (for example, $\cover$ for binary prediction), as in this case the regret is equalized over all inputs. However, the modification is necessary for a generic algorithm $\wcalg$ with (near optimal) worst-case regret guarantees, as such a $\wcalg$ may achieve very low regret on some inputs, and there is no way to match it on these.
 

==> arxiv/arxiv_body/skirental_arxiv.tex <==
\section{Improving the competitive ratio} \label{sec:SkiRental}

\begin{theorem}[Regret of $\bob$ with Randomized Thresholds]  \label{eq:SkiRentalRegret}
      Let $\wcalg$ have worst-case regret $g(n)$ over all inputs, and define cumulative density function $F_n(x) = \frac{e^{x/g(n)}-1}{e-1}$ for $x\in [0,g(n)]$. Now suppose we sample $\theta\sim F_n$, i.e., given $U\sim\text{Uniform}[0,1]$, we set
      \begin{align*}
      \theta=g(n)\ln(1+(e-1)U)
      \end{align*}
      Then the $\bob$ policy (\cref{metaalg:2approx}) with random threshold $\theta$ and policy $\wcalg$ has regret 
    \begin{align} 
    \label{eq:eApproxReg}
        \E_{\theta}\left[\Reg(\bob, \ell^n)\right] \le \frac{e}{e-1} \min\{\Reg(\ftl,\ell^n),g(n)\} + 1.
    \end{align}
\end{theorem}


The algorithm and proof follows a similar approach as that of the classical randomized algorithm for ski-rental~\cite{karlin1994competitive}
\begin{proof}
For a given sequence of loss functions $\ell^n$, we use the shorthand notation $r= \Reg(\ftl,\ell^n)$ and $g=g(n)$.
Also, for our given choice of cdf $F_n$, the corresponding pdf is given by $f(z) = \frac{e^{z/g}}{g(e-1)}$ for $z\in[0,g]$. 
As before, let $\tau \defeq \min_{1 \le t \le n-1} \ftlsum_t > \theta$ be the (random) round where $\bob$ switches from $\ftl$ to $\wcalg$ (with $\tau=n$ if it never switches). Then we have
\begin{align*}
\frac{\Reg(\bob,\ell^n)}{\min\{\Reg(\ftl,\ell^n),g(n)\}}\leq \begin{cases} 
   \frac{\theta + g}{\min\{r,g\}} & \text{if } \tau < n \\
   1       & \text{if } \tau = n
  \end{cases}
\end{align*}
where the second case follows from the fact that $\theta\in[0,g]$, and hence if we never switch, then $r\le g(n)$. 
Taking expectation over $\theta$, we have
\begin{align*}
\frac{\E_{\theta}\left[\Reg(\bob,\ell^n)\right]}{\min\{\Reg(\ftl,\ell^n),g\}}\le 
\begin{cases} 
   \int_0^r   \frac{x + g}{r}f(x)dx + 1 - F(r)  & \text{if } r \le g \\
   \int_0^g   \frac{x + g}{g}f(x)dx        & \text{if } r > g
  \end{cases}
\end{align*}
Let $\phi(z) \defeq  \int_0^z \frac{(x + g)}{z}f(x)dx + 1 - F(z) $ for $z\in[0,g]$; then $\frac{\E_{\theta}\left[\Reg(\bob,\ell^n)\right]}{\min\{\Reg(\ftl,\ell^n),g\}} \leq \max_{z\in[0,g]}\phi(z)$. Moreover, we can differentiate to get $z^2\phi'(z)= gzf(z) - \int_0^z(x + g)f(x)dx$. Substituting our choice of $f$ in this expression, we get
\begin{align*}
\frac{z^2d\phi(z)}{dz} &= \frac{ze^{z/g}}{(e-1)} - \int_0^z(x + g)\frac{e^{x/g}}{g(e-1)}dx
=\frac{ze^{z/g} - g\int_0^{z/g}(w + 1)e^{w}dw}{(e-1)}=0
%\\&=\frac{ze^{z/g} - g(ze^{z/g}/g)}{(e-1)} = 0
\end{align*}
Thus, $\phi(z)$ is constant for all $z\in[0,g]$, and moreover, $\phi(g) = \frac{1}{g(e-1)}\int_0^g(1+x/g)e^{x/g}dx = \frac{e}{e-1}$.
\end{proof}


\begin{remark}[Optimality for restricted class of algorithms] \label{rem:SkiRentalLB}
    
\end{remark}
